Research and development in cylindrical triple-GEM detector with $\mu$TPC readout for the BESIII experiment

The third generation of the Beijing Electron Spectrometer, BESIII, is an apparatus for high energy physics research. The hunting of new particles and the measurement of their properties or the research of rare processes are sought to understand if the measurements confirm the Standard Model and to look for physics beyond it. The detectors ensure the reconstruction of events belonging to the sub-atomic domain. The operation and the efficiency of the BESIII inner tracker is compromised due to the the radiation level of the apparatus. A new detector is needed to guarantee better performance and to improve the physics research. A cylindrical triple-GEM detector (CGEM) is an answer to this need: it will maintain the excellent performance of the inner tracker while improving the spatial resolution in the beam direction allowing a better reconstruction of secondary vertices. The technological challenge of the CGEM is related in its spatial limitation and the needed cylindrical shape. At the same time the detector has to ensure an efficiency close to 1 and a stable spatial resolution better than 150 $\mu$m, independently from the track incident angle and the presence of 1 T magnetic field. In the years 2014-2018 the CGEM-IT has been designed and built. Through several test beam and simulations the optimal configuration from the geometrical and electrical points of view has been found. This allows to measure the position of the charged particle interacting with the CGEM-IT. Two algorithms have been used for this purpose, the charge centroid and the $\mu$TPC, a new technique introduced by ATLAS in MicroMegas and developed here for the first time for triple-GEM detector. A complete triple-GEM simulation software has been developed to improve the knowledge of the detection processes. The software reproduces the CGEM-IT behavior in the BESIII offline software.

==> 00_introduction.tex <==
INTRODUCTION
\section{Introduction}

==> biblio_00_introduction.tex <==
\begin{thebibliography}
~Bibliography
\end{thebibliography}

==> ciao.tex <==
Ciao
